Importance Sampling and Adjoint Hybrid Methods in Monte Carlo Transport with Reflecting Boundaries

Adjoint methods form a class of importance sampling methods that are used to accelerate Monte Carlo (MC) simulations of transport equations. Ideally, adjoint methods allow for zero-variance MC estimators provided that the solution to an adjoint transport equation is known. Hybrid methods aim at (i) approximately solving the adjoint transport equation with a deterministic method; and (ii) use the solution to construct an unbiased MC sampling algorithm with low variance. The problem with this approach is that both steps can be prohibitively expensive. In this paper, we simplify steps (i) and (ii) by calculating only parts of the adjoint solution. More specifically, in a geometry with limited volume scattering and complicated reflection at the boundary, we consider the situation where the adjoint solution "neglects" volume scattering, whereby significantly reducing the degrees of freedom in steps (i) and (ii). A main application for such a geometry is in remote sensing of the environment using physics-based signal models. Volume scattering is then incorporated using an analog sampling algorithm (or more precisely a simple modification of analog sampling called a heuristic sampling algorithm) in order to obtain unbiased estimators. In geometries with weak volume scattering (with a domain of interest of size comparable to the transport mean free path), we demonstrate numerically significant variance reductions and speed-ups (figures of merit).

==> makefile <==
### Makefile for backing up all *.tex files in current directory to ./backup/backup.tar.gz ##

TIMESTAMP = $(shell date +%F_%H%M)

############################################################################
#The target "backup" creates and logs backups.
backup: copytobackup zipandname logbackup

#firstbackup is what you shouuld run the very first time you create backups.  It creates the backup directory and the logfile.
firstbackup: makebackupdirectory copytobackup zipandname makelogfile logbackup
############################################################################
#
copytobackup:
	cp *.tex backup/

# zipandname zips up all tex files into one archive.
zipandname:
	tar --remove-files -cvzf backup/zipfile backup/*.tex; mv backup/zipfile backup/${TIMESTAMP}.tar.gz

# Log version notes for the most recent version
logbackup:
	echo "\n">>backup/backup.log; echo ${TIMESTAMP}>>backup/backup.log; echo "\nEnter a note for archive.  Hit <CR> then ^D when done."; cat >>backup/backup.log

#
makebackupdirectory:
	mkdir backup

#
makelogfile:
	echo "Log of all backups of the project">>backup/backup.log; echo "~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~">>backup/backup.log

# Unzipbackup unzips the archive of all backup files, which is created with the target zipbackup.
unzipbackup:
	tar -xvzf backup/backup.tar.gz ;  rm backup/backup.tar.gz

# zipbackup zips all backup files into one file.  Not used when I'm working on the project.
zipbackup:
	tar --remove-files -cvzf backup/backup.tar.gz backup/* 
	
#mv zipfile $(date +%F_%R)  --remove-files
#	tar --remove-files -cvzf backup/zipfile backup/*.tex; mv backup/zipfile backup/$(date +%F_%R).tar.gz

